Two monads for graphs

An introduction to algebras for graphs, based on Courcelle's algebras of hyperedge replacement and vertex replacement. The paper uses monad notation.

==> algebraic-proof.tex <==

\subsubsection{An algebraic proof}
\label{sec:algebraic-proof-of-recognisability}
We now give a second  proof  of the Recognisability Theorem, which is algebraic. Essentially, the Recognisability Theorem is a special case of a more general result, namely~\cite[Lemma 6.2]{Anonymous:2015vr}, which says that ``languages definable in \mso'' are necessarily recognisable, under a suitable abstract notion of ``language definable in \mso''. To get the Recognisability Theorem from~\cite[Lemma 6.2]{Anonymous:2015vr}, we need to: (a) prove that the definition of \msotwo from Definition~\ref{def:msotwo} matches the abstract definition; and (b) overcome a mistake in the proof of~\cite[Lemma 6.2]{Anonymous:2015vr}, by showing that an additional assumption which was incorrectly omitted from~\cite{Anonymous:2015vr} is indeed satisfied\footnote{This mistake  was pointed out by Julian Salamanca. The proof of Lemma 6.2 in~\cite{Anonymous:2015vr} requires an additional assumption, namely that there is a distributive law of the monad over powerset.} Since the proof of Lemma 6.2 from~\cite{Anonymous:2015vr} is short even after fixing the mistake, we present the full argument here.


\paragraph*{Variable-free version of \mso.} The proof of the Recognisability Theorem in this section is essentially and induction on formula size. Since subformulas can have free variables, and recognisable languages do not use variables, it is convenient to use a classical coding of formulas with free variables into languages, see e.g.~\cite[p.~396]{Thomas:1990tw}. 

\begin{definition}[A variable-free version of \mso]\label{def:abstract-mso}
Define $\Ll$ to be the least class $\Ll$ of languages with the following properties:
\begin{enumerate}
 	\item For every  ranked set $\Sigma$ and $(a,i),(f,j) \in [\Sigma]$, the following language is in~$\Ll$:
\begin{align*}
\set{ G \in \hmonadzero \Sigma : \text{there exist hyperedges $e,f$ with labels $a,b$ that satisfy $e[i]=f[j]$}}	
\end{align*}
\item For every ranked set $\Sigma$, $a \in \Sigma$ and $m \in \Nat$, the following language is in $\Ll$:
\begin{align*}
\set {G \in \hmonadzero \Sigma. : \text{the number of hyperedges with label $a$ is divisible by $m$}}	
\end{align*}
\item $\Ll$ is closed under (finite) union and complementation;
	\item $\Ll$ is closed under images and pre-images under functions of the form 
\begin{align*}
\hmonad f : \hmonad \Sigma \to \hmonad \Gamma \qquad \text{for some }f : \Sigma \to \Gamma.	
\end{align*}
\end{enumerate}
\end{definition}

The following lemma shows that the above closure properties are sufficient to describe all of counting \mso. The basic idea is that the predicates correspond to the languages in items 1 and 2, and the  logical connectives correspond to closure operations in items 3 and 4  (with existential quantification being projection). The converse inclusion in  the lemma below is also true, but we only prove the inclusion that is needed for the Recognisability Theorem.





\begin{lemma}\label{lem:mso-to-lang}
Every language definable in counting \mso  belongs to $\Ll$.
\end{lemma}
\begin{proof}[Sketch]
Consider a sentence $\varphi$ of counting \mso, which defines a language of hypergraphs over a ranked alphabet $\Sigma$. Let $\psi$ be a subformula of $\varphi$. Let $\Xx$ be the free variables of  $\psi$. Some of these variables are first-order variables, and some of these variables are second-order variables.
Define 
\begin{align*}
\Sigma \times \powerset \Xx
\end{align*}
 to be the ranked alphabet which consists of one copy of $\Sigma$ for each subset of free variables in $\psi$. For a hypergraph
\begin{align*}
G \in \hmonad (\Sigma \times \powerset \Xx),
\end{align*}
we  define  a valuation $\eta_G$  of the free variables of $\psi$, which maps a second-order variable $X \in \Xx$ to the set of hyperedges that have $X$ in their variable, and which maps a first-order variable $x \in X$ to the unique hyperedges that has $x$ in its label (if the node is not unique, i.e.~there are zero or at least two hyperedges with $x$ in their label, then the valuation is undefined). The \emph{language} of $\psi$ is then defined to be the set of (rank zero) hypergraphs $G$ such that the valuation $\eta_G$ is defined and makes $\psi$ true in the hypegraph obtained from $G$ by projecting each label to $\Sigma$.  When $\psi$ is the entire sentence $\varphi$, this definition coincides with the usual notion of language.

By induction on the size of the subformula $\psi$, one shows that the language of very subformula is in the class $\Ll$. For atomic formulas, we use the languages in items 1 and 2; for the connectives we use the closure properties. 
%In the proof it is convenient to use the following language
%\begin{align*}
%\set{ G \in \hmonadzero \Sigma : \text{some  hyperedge has label $a$}}	
%\end{align*}
\end{proof}

\paragraph*{Proof of the Recognisability Theorem.} Thanks to the above lemma, in order to prove the Recognisability Theorem, it suffices to show that all languages in the class $\Ll$ are recognisable. We begin with the base languages.

\begin{lemma}
  The languages described in items 1 and 2 of Defintion~\ref{def:abstract-mso} are recognisable.
\end{lemma}
\begin{proof}
\begin{enumerate}
	\item Let $\Sigma$ and $(a,i)$ and $(f,j)$  be as in item 1 of Definition~\ref{def:abstract-mso}. Define an equivalence relation on $\hmonad \Sigma$ as follows. 
 \begin{align*}
G \sim H 	
\end{align*}
holds if (a) both $G$ and $H$ have the same rank, say $n$; and one of the following holds:
\begin{itemize}
	\item Both 
	\item For every $k \in \set{1,\ldots,n}$ and $\sigma \in \set{a,b}$, there is a hyperedge with label $\sigma$ in $G$ whose $k$-th vertex is 
\end{itemize}
On rank $n$, the universe of $\alga$ is equal to
\begin{align*}
\top + \set{a,b,\emptyset}^n.
\end{align*}
For a hypergraph $G \in \hmonad \Sigma$, its value under $h$ is defined as follows. If $G$ satisfies the condition from the language, then the value is $\top$. Otherwise, the value is the tuple
\begin{align*}
(A_1,\ldots,A_n)	
\end{align*}
such that 


\end{enumerate}
\end{proof}

To finish the proof of the Recognisability Theorem, we need to show that recognisable languages have the closure properties described in items 3 and 4 of Definition~\ref{def:abstract-mso}.
Recognisable languages are clearly closed under complementation -- it is enough to complement the accepting set. For union (or intersection), one uses Cartesian product of algebras, which preserves finiteness on every rank.  For inverse images under homomorphisms, we simply compose two homomorphisms. The hard case is images under homomorphisms; this case is proved below.

%\begin{definition}\label{def:graph-element} For a binary relation
%\begin{align*}
%R \subseteq \Sigma \times \Gamma 
%\end{align*}
%we define its lifting
%\begin{align*}
%\hmonad R \subseteq \hmonad \Sigma \times \hmonad \Gamma	
%\end{align*}
%to be the set of pairs $(G,H)$ such that there is some 
%\begin{align*}
%F \in \hmonad (\Sigma \times \Gamma)	
%\end{align*}
%which projects to  $G$ and $H$ the first and second coordinates, respectively.  
%\end{definition}
%An equivalent definition of $H \in G$ is that  there is some 
%\begin{align*}
%F \in \hmonad \set{(a,A) : a \in A \subseteq \Sigma})	
%\end{align*}
%which projects to $H$ and $G$  on the first and second coordinates respectively. The following lemma shows that there is a natural powerset operation on algebras.
%
 
\begin{lemma}
Recognisable languages are closed under  images  of functions of the form
\begin{align*}
\hmonad f : \hmonad \Sigma \to \hmonad \Gamma \qquad \text{for some }f : \Sigma \to \Gamma.
\end{align*}
\end{lemma}
\begin{proof}
Let $f$ be as in the statement of the lemma, and 
suppose that a language
\begin{align*}
L \subseteq \hmonadzero \Sigma	
\end{align*}
is recognised by a homomorphism
\begin{align*}
h : \hmonad \Sigma \to \alga	
\end{align*}
into an algebra that is finite on every rank. We will show that the image of $L$ under $\hmonad f$ is also recognisable. The algebra recognising the image will be obtained by applying a powerset construction to $\alga$. 

Let $A$ be the universe of the algebra $\alga$ and let $\pi$ be its product operation.   For 
\begin{align*}
H \in \hmonad A \qquad\text{and}\qquad  G \in \hmonad \powerset A	
\end{align*}
we write $H \in G$ if the two graphs have the same hyperedges, the same incidence relation, the same sources, and for every hyperedge $e$, the label of $e$ in $H$ is an element of the label of $e$ in $G$. Define (what will turn out to be an algebra) $\powerset \alga$ as follows. The universe is the powerset of the universe in $\alga$, and the product operation is defined by
\begin{align*}
 G  \mapsto \set{\text{product of $H$} : H \in G}.
\end{align*}
We will show below that (a) $\powerset \alga$ is an $\hmonad$-algebra; (b) the image of $L$ under $\hmonad f$ is recognised by this algebra. Since the powerset operation preserves finiteness, the statement of the lemma will follow.

\begin{claim}
	$\powerset \alga$ is an $\hmonad$-algebra.
\end{claim}
\begin{proof}
For a ranked set $A$, let 
\begin{align*}
\delta_A : \hmonad \powerset A \to \powerset \hmonad B	\end{align*}
 be the function defined by $G \mapsto \set{H : H \in G}$. In items 1 and 2 below we show that the family of functions $
\set{\delta_A}_A
$ is what is called in category theory \emph{a distributive law of the monad $\hmonad$ to the functor $\powerset$}.
\begin{enumerate}
	\item The family of functions $\set{\delta_A}_A$  is a natural transformation, in the sense of category theory, i.e.~for every rank-preserving function $f : A \to B$ the following diagram commutes:
\begin{align}
	\xymatrix{ 
	\hmonad \powerset A \ar[d]_{\hmonad \powerset f} \ar[r]^{\delta_A} & \powerset \hmonad A \ar[d]^{\powerset \hmonad A}\\
	\hmonad \powerset B \ar[r]_{\delta_B} & \powerset \hmonad B
	}
\end{align}
The commutativity of the above diagram says that there is no difference between: (a) relabelling the set on each hyperedge by $f$ and then choosing elements in the labels; and (b) first choosing elements in the labels, and then relabeling them according to $f$. 
\item For every ranked set $A$ the following diagram commutes
\begin{align}\label{eq:distributive-law}
\xymatrix{
\hmonad \hmonad \powerset A \ar[rr]^{\flatt_A} \ar[d]_{\hmonad \delta_A} & & \hmonad \powerset A \ar[d]^{\delta_A}\\
\hmonad \powerset \hmonad A \ar[r]^{\delta_{\hmonad A}} & \powerset \hmonad \hmonad A \ar[r]^{\powerset \flatt_A} & \powerset \hmonad A
}
\end{align}

\end{enumerate}

The rest of this proof has nothing to do with the specific monad $\hmonad$ and the powerset $\powerset$; it works for any distributive law of a monad over a functor. By unraveling the definition of the product operation in the algebra $\powerset \alga$, the  associativity axiom for an Eilenberg-Moore algebra says that the following diagram should commute:
\begin{align}\label{eq:em-powerset}
\xymatrix{
\hmonad \hmonad \powerset A \ar[rr]^{\flatt_A} \ar[d]_{\hmonad \delta_A} & & \hmonad \powerset A \ar[d]^{\delta_A}\\
\hmonad \powerset \hmonad A  \ar[d]_{\hmonad \powerset \pi} & & \powerset \hmonad A \ar[d]^{\powerset \pi}\\
\hmonad \powerset A \ar[r]_{\delta_A} & \powerset \hmonad A \ar[r]_{\powerset \pi} & \powerset A
}
\end{align}
Extend the above diagram as follows:
\begin{align}\label{eq:em-powerset-bis}
\xymatrix{
\hmonad \hmonad \powerset A \ar[rr]^{\flatt_A} \ar[d]_{\hmonad \delta_A} & & \hmonad \powerset A \ar[d]^{\delta_A}\\
\hmonad \powerset \hmonad A \ar[r]^{\delta_{\hmonad A}} \ar[d]_{\hmonad \powerset \pi} & \powerset \hmonad \hmonad A \ar[r]^{\powerset \flatt_A} \ar[d]_{\powerset \hmonad \pi}& \powerset \hmonad A \ar[d]^{\powerset \pi}\\
\hmonad \powerset A \ar[r]_{\delta_A} & \powerset \hmonad A \ar[r]_{\powerset \pi} & \powerset A
}
\end{align}
The upper rectangle commutes by the claim. The lower left rectangle commutes by naturality. This completes the proof of the claim. 
\end{proof}

\begin{claim}
	The image of $L$ under $\hmonad f$ is recognised by $\powerset \alga$.
\end{claim}
\begin{proof}
Define 
\end{proof}
\end{proof}






==> courcelle-rubbish.tex <==

\subsection{Recognisability equals definability for bounded treewidth}
\label{sec:courcelle-conjecture}


The key result in~\cite{Bojanczyk:2016wd} is  that an \mso transduction can compute tree decompositions for graphs of bounded treewidth; \mso transductions also play a key role in this section. Therefore,  we begin by introducing terminology for transductions.

\paragraph*{\mso transductions.}  For ranked sets $\Sigma$ and $\Gamma$, viewed as vocabularies for relational structures, define a \emph{transduction with input vocabulary $\Sigma$ and output vocabulary $\Gamma$}  to be any set of pairs 
\begin{align*}
  (\structa,\structb) \qquad \text{where $\structa,\structb$ are structures over vocabularies $\Sigma,\Gamma$, respectively}
\end{align*}
which is closed under isomorphism, i.e.~replacing either the first or second coordinate by an isomorphic structure does not affect memebership in the set. An \mso transduction is a special case of a transduction, which is definable using formulas of \mso, see~\cite[Definition 2.3]{Bojanczyk:2016wd} for the  definition used here.  We will be interested in \mso transductions that define binary relations on labelled hypergraphs, i.e.~\mso transductions of the form
\begin{align*}
  \Tt \subseteq \hmonadzero \Sigma \times \hmonadzero{\Gamma}.
\end{align*}
for some ranked sets $\Sigma$ and $\Gamma$.   For such a transduction and $\structa \in \hmonadzero{ \Sigma}$, we write $\Tt(\structa)$ for the set of $\structb$ which satisfy $(\structa,\structb) \in \Tt$. Note that the set $\Tt(\structa)$ need not contain exactly one element, it can be empty or contain more than two elements; this is why \mso transductions are sometimes called \emph{nondeterministic}.  

\paragraph*{Unranked unordered terms.}  Our  goal is to show -- using~\cite[Theorem 2.4]{Bojanczyk:2016wd} -- that there is a (nondeterministic) \mso transduction which maps hypergraphs of bounded treewidth to their tree decompositions. In the spirit of Theorem~\ref{thm:treewidth-grammar}, we view tree decompositions as terms using polynomials from the algebra $\hmonad \edgevoc$.   An important limitation  is that it is not enough to  produce terms (that represent tree decompositions) of bounded branching, e.g.~branching at most two. Intuitively speaking, the reason for using high branching is that if the input is an independent set like this:
\mypic{38}
then the tree decomposition produced by  an \mso transduction will look like this: 
\mypic{39}  
and not like this
\mypic{40}  
The issue is that the lower tree decomposition (and any other tree decomposition with bounded branching) would induce an ordering on the independent set, something which cannot be done in \mso. In  the proof of Theorem~\ref{thm:treewidth-grammar} we did not have this limitation, because we only cared about the existence of a tree decomposition, and it was not important that this tree decomposition would have to be produced using \mso. 


To deal with the issues described above, we use terms where the  operations have no order on children and the branching is not bounded. For such terms, nodes with more than two children will be labelled by associative commutative operations, as defined below.

\begin{definition}[Unordered unranked terms] 
%An \emph{associative commutative} operation over a set $A$ is a function 
%\begin{align*}
%f : A \times A \to A	
%\end{align*}
%which satisfies the following identities
%\begin{align*}
%\underbrace{f(a,b) = f(b,a)}_{\text{commutative}} \qquad \underbrace{f(a,f(b,c)) = f(f(a,b),c)}_{\text{associative}}.
%\end{align*}
%An associative and commutative operation can be extended multisets of arguments, as defined by 
%\begin{align*}
%f(a_1,\ldots,a_n) = f(a_1,f(a_2,\ldots,a_n)) \qquad f(a)=a.
%\end{align*}
	A polynomial in a $\hmonad$-algebra with universe $A$ is called \emph{associative commutative} if it is of the form 
	\begin{align*}
f : \slice A n \times \slice A n \to \slice A n	 
\end{align*}
for some rank $n$, and is associative and commutative in the usual sense.  
%For an associative acommutative polynomial $f$, we define
%\begin{align*}
%f^+ : \text{multisets over $\slice A n$}  \to \slice A n 
%\end{align*}
%
Define an \emph{unranked term over a $\hmonad$-algebra $\alga$} to be a tree (labelled, unranked and without an order on siblings, see Figure~\ref{fig:trees}) where every node is labelled by a polynomial in $\alga$  which has  either zero or one arguments, or has two arguments and is associative commutative.
\end{definition}
 The value   of an unranked term $t$ is defined in the natural way, by induction on the size of $t$: if  a tree has root label $f$ and $n$ children, then its value is defined to be
 \begin{align*}
f(\text{value of child $1$}, \ldots, \text{value of child $n$}).
\end{align*}
The above expression is undefined if either: (a) one of the children has undefined value; or (b) $f$ is a polynomial with $m \in \set{0,1}$ arguments but $n \neq m$; or (c) $f$  has two arguments and $n < 2$; or (d) some child produces a value whose  rank is different than the rank of the arguments of $f$.

 


\paragraph*{Computing tree decompositions with \mso transductions.}
The main technical result of this section, Theorem~\ref{thm:mso-transduction-treedecomp} below,   says that an \mso transduction can input a hypergraph and output an unranked term in the algebra $\hmonad \Sigma$ that produces it. When we talk about \mso transductions producing trees, we use the following representation of trees are relational structures: the  universe is the nodes of the tree, there  is a binary predicate for the parent relation, and there is a unary predicate for every label which selects nodes with that label.	

\begin{theorem}\label{thm:mso-transduction-treedecomp}
	For every $k \in \Nat$  there is a finite set $P$ of polynomials in $\hmonad \edgevoc$, which have zero or one arguments or are associative commutative,   
and a nondeterministic \mso transduction
	\begin{align*}
 \Tt \subseteq \set{(G,t) : 
 \begin{cases}
 \text{$G$ is a directed graph}\\
 \text{ 	$t$ is an unranked term with value $G$ that uses polynomials from $P$}
 \end{cases}
}
\end{align*}
such that for every graph $G$ with treewidth at most $k$, the set $\mathcal \Tt(G)$ is nonempty.
\end{theorem}




Before proving the above theorem, we use it to prove Theorem~\ref{thm:courcelle}. 


\begin{proof}[of Theorem~\ref{thm:courcelle}]
In the proof we use the following definition: a binary relation $R$ between relational structures and elements of some set $A$ is called \emph{definable in counting \mso} if for every $a \in A$, the set
\begin{align*}
R^{-1}(a) \eqdef \set{\structa : (\structa, a) \in R}	
\end{align*}
is definable in counting \mso. Suppose that a language $L$ of hypergraphs over $\Sigma$ is recognised by a homomorphism
\begin{align*}
 h : \hmonad \Sigma \to \alga
\end{align*}
where $\alga$ is finite on every rank. Our goal is to show that $h$, when viewed as a binary relation, is definable in counting \mso. This will imply that $L$ is definable in counting \mso, since  
\begin{align*}
L = \bigcup_{a \in h(L)} h^{-1}(a)	
\end{align*}
and the union is  finite, since it contains only elements of rank zero.

Apply Theorem~\ref{thm:mso-transduction-treedecomp}, yielding a finite set of polynomial operations $\Gamma$ and an \mso transduction $\Tt$. 
 Consider the following diagram, where dotted arrows are binary relations, and solid arrows are functions:
\begin{align*}
\xymatrix @C=2cm @R=2cm
{
&\text{hypergraphs over $\Sigma$ with treewidth $\le k$}
\ar@{.>}[d]^\Tt \ar@{^{(}->}[ddl]_{\text{id}} \ar@{.>}[ddr]^{h \circ \text{value} \circ \Tt}
\\
& \text{trees labelled by $\Gamma$} \ar[dl]^{\text{value}} \ar[dr]_{h \circ \text{value}}\\
\hmonad \Sigma \ar[rr]_{ h} & &  A
}	
\end{align*}
  The right and bottom small triangles commute by definition, while the  left small  triangle commutes by Theorem~\ref{thm:mso-transduction-treedecomp}. It follows that the big  triangle commutes (in particular, the right dotted line in the diagram can be made solid, because it is a composition of two functions).  The function $h \circ \text{value}$ is recognisable in the sense of functions from (unranked unordered) trees to a finite set, see~\cite[Section 5]{Courcelle:1990fj}, and therefore it is definable in counting \mso, see~\cite[Theorem 5.3]{Courcelle:1990fj}. The Backwards Translation Theorem~\cite[Theorem 7.10]{Courcelle:2012wq}  says that the composition of an \mso transduction with a relation definable in counting \mso gives a relation that is also definable in counting \mso, and therefore   $h \circ \text{value} \circ \Tt$ is definable in counting \mso. Since the diagram commutes, it follows that $h$, when restricted to arguments of rank zero, is also definable in counting \mso.
  \end{proof}

The rest of Section~\ref{sec:courcelle-conjecture} is devoted to proving  Theorem~\ref{thm:mso-transduction-treedecomp}, which says that an \mso transduction can compute a tree decomposition (represented as an unranked term). 
The theorem was proved for   graphs (not hypergraphs) in~\cite[Theorem 2.4]{Bojanczyk:2016wd}, so the proof below simply consists of adapting the result from~\cite{Bojanczyk:2016wd} to hypergraphs. We do the adaptation in three steps: (1) code a hypergraph as a graph; (2) compute the tree decomposition of the resulting graph; (3) convert this tree decomposition  into a tree that describes the original hyperegraph.


%For such a graph, we write
%\begin{align*}
%  v \stackrel a \to w
%\end{align*}
%if there is a hyperedge with label $a$ that goes from $v$ to $w$. 


We begin by defining the coding of hypergraphs as graphs, which we call \emph{binarisation}. When speaking of graphs in this proof, we use  \emph{directed graphs}: this is the special case of   hypergraphs where all hyperedges have rank two and there multiple edges are forbidden, i.e.~no two hyperedges (even with different labels) have the same source and target.  Note that hypergraphs have labelled hyperedges, and therefore our directed graphs have labelled edges.


\begin{definition}[Binarisation]
	For a hypergraph $G$ over $\Sigma$, define its \emph{binarisation} to be  the following  edge  coloured directed graph.   The vertices of the binarisation are the vertices plus   hyperedges in $G$. The edge colours are natural numbers (up to the maximal rank of $\Sigma$). The edges of the binarisation are defined by
	\begin{align*}
  e \stackrel i \to v  \qquad \text{iff} \qquad \text{$e$ is a hyperedge and $v$ is a vertex with $e[i]=v$}
\end{align*}	
\end{definition}

The following result shows that binarisation has little effect on  treewidth.


\begin{fact}\label{fact:binarisation}
	If a hypergraph  has treewidth $k$, then  its binarisation has treewidth at most $\max(k, \text{maximal rank of a hyperedge})$.
\end{fact}
\begin{proof} Let $t$ be a tree decomposition of a hypergraph $G$. For each hyperedge $e$ of $t$, find a node $x$ of the tree decomposition whose bag contains all vertices adjacent to $e$. Add a child node to $x$, whose bag contains a vertex that represents $e$ plus all the vertices adjacanet to $e$.  
\end{proof}

We have defined (edge labelled) directed graphs as a special case of hyperegraphs, and so we can apply the encoding as relational structures that was defined for hypergraphs in Definition~\ref{def:relational-encoding}. Therefore it makes sense to talk about \mso transductions that input or output binarisations. It remains to describe how tree decompositions are represented as relational structures. The following definition is adapted from~\cite[page 2]{Bojanczyk:2016wd}.

\begin{definition}[Tree decompositions as relational structures]\label{def:tree-decompositions-as-relational-structures}
Let $G$ be a coloured undirected graph. We view a tree decomposition of $G$ as a relational structure as follows. The universe of the structure is the disjoint union
\begin{align*}
  \text{edges of $G$} \quad + \quad   \text{vertices of $G$} \quad + \quad   \text{nodes of $t$}.
\end{align*}
There are three binary predicates which describe: (a)  the incidence relation betwen vertices and edges; (b)  the parent relation on nodes; and (c) the bag membership relation between vertices and nodes. For every colour  $a$ used in the graph, there is a unary predicate which selects vertices with colour $a$.	
\end{definition}


By composing the three transductions $\Aa,\Bb, \Cc$ in the following lemma, and using Fact~\ref{fact:binarisation}, we get Theorem~\ref{thm:mso-transduction-treedecomp}. Since \mso transductions are closed under composition, in order to prove Theorem~\ref{thm:mso-transduction-treedecomp}, it remains to prove the lemma.

\begin{lemma}\label{lem:abc-transductions}
Let $k \in \Nat$ and let $\Sigma$ be finite ranked set. Then
\begin{enumerate}
	\item the following is an \mso transduction
	\begin{align*}
 \Aa  =  \set{(G,G') : 
 \begin{cases}
 \text{$G$ is a hypergraph over $\Sigma$}\\
 \text{$G'$ is its binarisation}
 \end{cases}
};
\end{align*}
\item there is some $k' \in \Nat$ and an \mso transduction
	\begin{align*}
 \Bb \subseteq \set{(G',t) : 
 \begin{cases}
 \text{$G'$ is an directed graph with vertices labelled by $\Delta$}\\
 \text{ 	$t$ is a tree decomposition of $G$ of width at most $k'$}
 \end{cases}
}
\end{align*}
such that for every  $G'$ of treewidth at most $k$, the set $\mathcal \Bb(G)$ is nonempty;
\item for every $k' \in \Nat$ there is a
	a finite set $\Gamma$ of polynomial operations in $\hmonad \Sigma$ and an \mso transduction
	\begin{align*}
 \Cc \subseteq \set{(t,s) : 
 \begin{cases}
 \text{$t$ is a  tree decomposition of the binarisation of some hypergraph $G$ over $\Sigma$}\\
 \text{$s$ is a tree labelled by $\Gamma$ that has value $G$}
 \end{cases}
}
\end{align*}
such that for every $t$ of width at most $k'$, the set $\Cc(t)$ is nonempty.
\end{enumerate}

\end{lemma}



%
%\begin{proof}
%
%\begin{enumerate}
%	\item For $k \in \set{1,2,\ldots}$ define $\alga_k$ to be following algebra. The universe $A$ is defined to be the ranked set which has a copy of  $\set{0,1,\ldots,n-1}$ on every rank. The product operation
%	\begin{align*}
%\pi_k: \hmonad 	A \to A
%\end{align*}
%maps a sourced hypergraph to the sum modulo $k$ of all labels in its hyperedges. It is not hard to see that this operation is associative.
%\item 
%\end{enumerate}
%
%	\begin{itemize}
%	\item For every $n \in \Nat$, every finite alphabet $\Sigma$, and every $R \in \Sigma$, the following set of hypergraphs over $\Sigma$ is recognised by a $\hmonad$-algebra that is finite on every rank:  
%	\begin{align*}
%\set{ \structa : \text{the number of hyperedges with label $R$ is divisible by $n$}}	
%\end{align*}
%
%	\item For  every finite ranked alphabet $\Sigma$, every $R,S \in \Sigma$, the following set of hypergraphs over $\Sigma$ is recognised by a $\hmonad$-algebra that is finite on every rank:  
%	\begin{align*}
%\set{ \structa : \text{there exist hyperedges $e_1,e_2$ with labels $R_1,R_2$ such that  $e_1[i_1]=e_2[i_2]$ }}	
%\end{align*}
%
%		\item Recognisable languages are closed under Boolean combinations. Indeed, if a language is recognised by some homomorphism, then also the complement of the language is recognised by the same homomorphism, only the accepting set needs to be changed. For union and intersection, one uses Cartesian product: if  $L_1,L_2$ are recognised by homomorphisms
%\begin{align*}
%h_i : \hmonad \to \alga_i \qquad \text{for $i \in \set{1,2}$}
%\end{align*}
%then their union and intersection are recognised by the homomorphism
%\begin{align*}
%(h_1,h_2) : \hmonad \Sigma \to  \alga_1 \times \alga_2
%\end{align*}
%\end{itemize}
%\end{proof}
%
%
%



==> general-mso.tex <==
\section{Generic results on \mso}

\subsection{Compositional relational encodings}

\begin{definition}[Compositional relational encoding]\label{def:compositional-relational-encoding} Fix a category of sorted sets.
Let $\tmonad$ be a monad in this category and let $\Sigma$ be a sorted set (i.e.~an object in the category). A \emph{compositional relational encoding} is defined to be a function
	\begin{align*}
\struct : \tmonad \Sigma \to \text{structures over $\underline \Sigma$}
\end{align*}
(with the domain viewed as a set, not a sorted set) which maps each element of  $\tmonad \Sigma$ to a structure over some fixed relational  vocabulary $\underline \Sigma$ such that the following property is satisfied. For every sorted set $X$ and every $G \in \tmonad X$ there is a reduction 
\begin{align*}
  f : (\text{structures over $\underline \Sigma$})^X \to \text{structures over $\underline \Sigma$}
\end{align*}
which makes the following diagram commute
\begin{align*}
\xymatrix{
(\hmonad \Sigma)^X \ar[rr]^{\struct^X} \ar[d]_{\eta \mapsto \hmonad \eta (G)} & & (\text{structures over $\underline \Sigma$})^X \ar[dd]^{f}\\
\hmonad \hmonad \Sigma \ar[d]_{\flatt \Sigma} \\
\hmonad \Sigma \ar[rr]_{\struct} & &  \text{structures over $\underline \Sigma$}
}
\end{align*}
A compositional relational encoding is called \emph{additive} if the reduction $f$ is required to be additive.

\end{definition}

\begin{lemma}\label{lem:}
If $r$ is a quantifier rank and 
	\begin{align*}
\struct : \tmonad \Sigma \to \text{structures over $\underline \Sigma$}
\end{align*}
is a compositional relational encoding, then 
 the equivalence  relation 
\begin{align*}
\text{$G,H$ have the same sort and  satisfy $\struct G \equiv_r \struct H$}
\end{align*}
is a congruence in the algebra $\tmonad \Sigma$. If the encoding is additive, then also
\begin{align*}
\text{$G,H$ have the same sort and  satisfy $\struct G \cmsoequiv_{r,M} \struct H$}
\end{align*}
\end{lemma}
\begin{proof}
\end{proof}



==> grammars.tex <==
\section{Grammars}
We now define grammars which work inside an arbitrary algebra over an arbitrary monad, under the assumption that the underlying category is a category of multisorted sets. 

\begin{definition}[Grammar] \label{def:grammar} Consider a category of multisorted sets. Let $\tmonad$ be a monad in this category,  and let  $\alga$ be an algebra over  $\tmonad$. 
	A \emph{grammar} over $\alga$ consists of:
	\begin{enumerate}
		\item a (sorted) set $\Sigma$ of terminals;
		\item a (sorted) set $X$ of nonterminals;
		\item  a distinguished \emph{starting} nonterminal $x_0 \in X$;
		\item a  finite set of rules contained in
		 \begin{align*}
\coprod_{Y \subseteq X} X \times \alga[Y]	
\end{align*}

	\end{enumerate}
\end{definition}
We write a rule as $x \to f$ where $x$ is a nonterminal and $f$ is a polynomial operation in $\alga[Y]$ for some $Y \subseteq X$.

%A solution of the grammar is defined to be any function
%\begin{align*}
%\eta : X \to \powerset (A)
%\end{align*}
%such that every rule $x \to p$ satisfies
%\begin{align*}
%	\sem p (\eta) 
%\end{align*}

\begin{myexample}\label{ex:exponentiating-grammar}
	Suppose that the monad is the monad of finite words over the category of finite sets.  Here is an example of an grammar over the algebra $\set{a}^*$. There is one nonterminal $x$, which is also the starting nonterminal, and the rules are
	\begin{align*}
x \to a \qquad x \to xx.
\end{align*}
As we will see below this grammar generates all words whose length is of the form $2^n$. This example is meant to highlight the difference with usual context-free gramars, where multiple appearances of the same nonterminal in a rule are treated as independent.
\end{myexample}

A grammar generates a language, which is a subset of the universe of $\alga$ that has only elements of the same rank as the starting nonterminal. To define the generated language, we use derivation trees (an alternative approach would use least fixpoints of operations on tuples of languages). 
Consider a tree where each node is labelled by a rule of the grammar. If a node in  tree is labelled by a rule $x \to f$, then we call $x$ the nonterminal of the node, and we call $f$ the \emph{right hand side} of the node. Such a tree is called a \emph{derivation} if for every node with right hand side $f$, the node has exactly one child for  each variable $x$ used by $f$,  and the nonterminal of that child is $x$. In particular, if $f$ uses no variables, i.e.~$f \in \alga[\emptyset]$ then the node has  no children.  Here is a picture of a derivation tree for the grammar from Example~\ref{ex:exponentiating-grammar}:
\mypic{24}

The \emph{yield} of a derivation is an element of the universe $\alga$  defined as follows by induction on the depth of the tree. Suppose that $t$ is a derivation whose root has  right hand side  $p$, and let $Y \subseteq X$ be the variables of  $f$. The yield of $t$ is obtained by  applying $f$ to the valuation
\begin{align*}
y \in Y \quad \mapsto \quad \text{yield of the child of $t$ corresponding to $y$}.
\end{align*}
The language generated by a grammar consists of the yields of derivation where the nonterminal of the root is the starting nonterminal.

\subsection{Hyperedge replacement grammars}




\begin{myexample}\label{ex:balanced-trees}	Consider grammar over $\hmonad \Sigma$ where $\Sigma$ has one binary letter which we draw like this:
	\mypic{19}
	Hypergraphs over this set of labels are graphs (directed and with multiple edges).
	The grammar has one nonterminal of arity one, which we draw like this:
	\mypic{14}
	The grammar has two rules. The first rule\footnote{According to Definition~\ref{def:grammar}, a  polynomial (e.g.~a polynomial defining the right hand side in a rule of a grammar)  with variables $X$ in an algebra of the form $\hmonad \Sigma$ is an element of 
\begin{align*}
\hmonad (\hmonad \Sigma + X)	
\end{align*}
By abuse of notation, to define polynomials we will use  elements of 
\begin{align*}
 \hmonad (\Sigma + X).
\end{align*}
Formally speaking,  to treat such elements as polynomials,  we would need to replace each element of $\Sigma$ by its corresponding units.
}
	 says that the nonterminal can generate a sourced graph with one isolated node that is the source:
	\mypic{20}
	The second rule  allows us to combine two copies of an already generated graph:
	\mypic{12}
	Note that the two appearances of the same nonterminal are going to be substituted with the same sourced graph -- this is the same phenomenon as in the grammar from Example~\ref{ex:exponentiating-grammar}. Therefore, the  language generated by the grammar above  consists of unary sourced graphs which are  balanced binary trees, with edges directed toward the root, and where the root is the source.
\end{myexample}

\begin{myexample}\label{ex:unbalanced-trees}
	We now define a grammar which generates all trees (viewed as  sourced directed graphs of rank one, where source 1 is the root, and where the edges are directed toward the root). Unlike in Example~\ref{ex:balanced-trees}, we will generate trees that are not necessarily balanced. The grammar has two nonterminals of rank one, called yellow and orange, which we draw like this:
	\mypic{16}
	As  in Example~\ref{ex:balanced-trees}, we have a rule that generates isolated nodes:
	\mypic{20}
	We can also add edges to sourced graphs  generated by the yellow nonterminal:
	\mypic{17}
	Finally, we want to say that any two (possibly distinct) sourced graphs  generated by the yellow nonterminal can be fused along their sources. To model the fact that possibly distinct sourced graphs are used,  we introduce another nonterminal (orange) and use the following two rules:
	\mypic{18}
	The first rule above says that the orange nonterminal can generate anything that is generated by the yellow one (the right hand side of the first rule is a unit). In the second rule, since two different nonterminals -- yellow and orange are used -- they can be evaluated with different graphs. It is not hard to see that this grammar generates exactly all finite trees.
	\end{myexample}
	
	\begin{myexample}
		Here is a grammar that generates all directed cycles of length at least two. There are two nonterminals: the starting nonterminal (yellow) has rank zero, the other nonterminal (orange) has rank two. Here are the rules:
		\mypic{22}
	\end{myexample}

